LogiGAN: Learning Logical Reasoning via Adversarial Pre-training

We present LogiGAN, an unsupervised adversarial pre-training framework for improving logical reasoning abilities of language models. Upon automatic identifying logical reasoning phenomena in massive text corpus via detection heuristics, we train language models to predict the masked-out logical statements. Inspired by the facilitation effect of reflective thinking in human learning, we analogically simulate the learning-thinking process with an adversarial Generator-Verifier architecture to assist logic learning. LogiGAN implements a novel sequential GAN approach that (a) circumvents the non-differentiable challenge of the sequential GAN by leveraging the Generator as a sentence-level generative likelihood scorer with a learning objective of reaching scoring consensus with the Verifier; (b) is computationally feasible for large-scale pre-training with arbitrary target length. Both base and large size language models pre-trained with LogiGAN demonstrate obvious performance improvement on 12 datasets requiring general reasoning abilities, revealing the fundamental role of logic in broad reasoning, as well as the effectiveness of LogiGAN. Ablation studies on LogiGAN components reveal the relative orthogonality between linguistic and logic abilities and suggest that reflective thinking's facilitation effect might also generalize to machine learning.

==> 05_backup_results.tex <==
\section{Experiments} \label{sec:exp}


\subsection{Experimental Results}
% Table generated by Excel2LaTeX from sheet '主实验'
\vspace{-2mm}
\begin{table}[htbp]
  \centering
  \caption{Main results of LogiGAN on 12 downstream tasks (\textit{development sets} judgement).}
  \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{ccccccccc}
    \toprule
    \multicolumn{9}{c}{Multiple Choice \& Classification Datasets} \\
    \midrule
    \multicolumn{2}{c} {Models\,/\,Dataset} & ReClor & LogiQA & RACE  & DREAM & ANLI  & MuTual & \multicolumn{1}{c}{Avg.} \\
    \multicolumn{2}{c}{\small Metrics} & {\small {\small $Acc$}}   & {\small {\small $Acc$}}   & {\small {\small $Acc$}} & {\small {\small $Acc$}} & {\small {\small $Acc$}} & {\small {\small $Acc$}} &  \\
    \midrule
    \multicolumn{2}{c}{Vanilla T$5_{~base}$} & $35.20$ & $27.19$ & $63.89$ & $59.36$ & $44.10$ & $67.38$ & $49.52$ \\
    \multicolumn{2}{c}{LogiGAN$_{~base}$ (ss)} & $40.20$ & $34.72$ & $67.13$ & $63.38$ & $49.50$ & $69.41$ & $54.06$\\
    \multicolumn{2}{c}{LogiGAN$_{~base}$ (ss+es)} & $40.00$ & $37.02$ & $67.27$ & $63.73$ & $49.70$ & $69.98$ & $54.62$\\
    \midrule
    \multicolumn{2}{c}{Vanilla T$5_{~large}$} & $50.40$ & $38.56$ & $78.99$ & $78.98$ & $58.00$ & $76.41$ & $63.56$\\
    \multicolumn{2}{c}{LogiGAN$_{~large}$} & $54.80$ & $40.55$ & $80.67$ & $81.42$ & $63.50$ & $77.88$ & $66.47$\\
    \midrule
    \multicolumn{9}{c}{Generation Datasets} \\
    \midrule
    \multicolumn{2}{c} {Models\,/\,Dataset} & QuoRef & HotpotQA & NarrativeQA & TellMeWhy & SAMSum & XSum & \multicolumn{1}{c}{Avg.} \\
    \multicolumn{2}{c}{\small Metrics} & {\small {\small EM\,/\,F$_1$}} & {\small {\small EM\,/\,F$_1$}}  & {\small Rouge$_L$} & \small Rouge$_L$ & {\small Rouge$_L$} & {\small Rouge$_L$} & \\
    \midrule
    \multicolumn{2}{c}{Vanilla T$5_{~base}$}  & $70.76$\,/\,$74.58$ & $61.11$\,/\,$74.86$ & $48.11$ & $30.03$ & $39.32$ & $29.14$ & $36.65$\\
    \multicolumn{2}{c}{LogiGAN$_{~base}$ (ss)} & $75.02$\,/\,$78.68$ & $62.68$\,/\,$76.14$ & $49.44$ & $31.18$ & $39.92$ & $30.26$ & $37.70$\\
    \multicolumn{2}{c}{{LogiGAN$_{~base}$} (ss+es)} & $74.94$\,/\,$78.40$ & $62.80$\,/\,$76.18$ & $49.46$ & $31.15$ & $40.21$ & $30.27$ & $37.77$ \\
    \midrule
    \multicolumn{2}{c}{Vanilla T$5_{~large}$} & $80.06$\,/\,$83.25$ & $66.11$\,/\,$79.80$ & $51.09$ & $31.42$ & $41.40$ & $31.58$ & $38.87$ \\
    \multicolumn{2}{c}{LogiGAN$_{~large}$} & $81.92$\,/\,$85.25$ & $67.04$\,/\,$80.36$ & $51.79$ & $32.72$ & $43.13$ & $33.49$ & $40.28$ \\
    \bottomrule
    \end{tabular}}
  \label{tab:main}%
  \vspace{-2mm}
\end{table}%
As presented in Table \ref{tab:main}, 
both base and large size PLMs further pre-trained with LogiGAN surpass their vanilla baselines across both discriminative and generative task formats, through a wide scope of downstream tasks requiring general reasoning abilities. 
We can make the following observations:
Among all observed improvements, those on tasks with particular emphasis on logic (ReClor, LogiQA, and ANLI) are most noticeable.
These positive results manifest the effectiveness of LogiGAN in injecting logic ability into PLMs, while testifying to our primary hypothesis that logic ability is fundamental to general reasoning as well.
This conclusion answers the two questions in the intro section \footnote{Is logic ability obtained for free from MLM? Could it be further learned
beyond language acquisition?}, suggesting that randomized MLM pre-training might fall short in endowing language models with logic ability, and a logic-targeted pre-training approach like LogiGAN may further assist logic learning beyond language acquisition.
Furthermore, extra retrieved pseudo-statements (ss+es) bring some additional performance improvement compared with the pure self-sampling (ss) LogiGAN variant, revealing the important role of pseudo-statements' \textit{diversity} in adversarial training.

\subsection{Ablation Study and Analysis}

% Table generated by Excel2LaTeX from sheet 'Ablation'

Observing the apparent performance enhancement, we now aim at pinpointing the truly functional components of LogiGAN through ablation studies and deriving the origins of observed improvements.
For fair comparison purposes, we hold all pre-training and downstream settings (including hyper-parameters, implementation designs, and evaluations) unchanged from full LogiGAN.
All variations are initialized from T$5_{base}$, and we report performance variance on $7$ datasets. 

\definecolor{Gray}{gray}{0.9}
\begin{table}[htbp]
  \centering
  \caption{Ablation Results on $7$ datasets. The last column shows average performance variance, along with relative percentage improvement against vanilla T$5_{base}$ as the baseline.}
  \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{cccccccccc}
    \toprule
    \multicolumn{2}{c}{Models\,/\,Dataset} & ReClor & LogiQA & RACE  & DREAM & ANLI & QuoRef & NarrativeQA &{---} \\
    \multicolumn{2}{c}{\small Metrics} & {\small $Acc$}   & {\small $Acc$}   & {\small $Acc$}   & {\small $Acc$} & {\small $Acc$} & {\small EM\,/\,F$_1$} & {\small Rouge$_L$} & {\small Average} \\
    \midrule
    \multicolumn{2}{c}{Vanilla T5$_{~base}$} & $35.20$  & $27.19$ & $63.89$ & $59.36$ & $44.10$ & $70.76$\,/\,$74.58$ & $48.11$ & $49.80_{(+0.0\%)}$ \\
    \rowcolor{Gray}
    \multicolumn{2}{c}{LogiGAN$_{~base}$ (ss+es)} & $40.00$  & $37.02$ & $67.27$ & $63.73$ & $49.70$ & $74.94$\,/\,$78.40$ & $49.46$ & $54.59_{(+9.6\%)}$ \\
    \midrule
    \multicolumn{2}{c}{I. Random Sentence} & $36.00$ & $30.56$ & $61.26$ & $58.15$ &  $45.40$ & $70.96$\,/\,$74.50$ & $48.38$  & $50.10_{(+0.6\%)}$ \\
    \multicolumn{2}{c}{II. MLE Logic Pre-train } & $38.80$  & $35.02$ & $64.55$ & $61.71$ & $46.00$ & $73.61$\,/\,$76.96$ & $49.30$ & $52.71_{(+5.9\%)}$ \\
    \multicolumn{2}{c}{III. Iterative Multi-task} & $37.20$  & $34.25$ & $64.01$ & $62.06$ & $46.20$ & $71.67$\,/\,$75.14$ & $49.15$ & $52.08_{(+4.6\%)}$  \\
    \bottomrule
    \end{tabular}}
  \label{tab:ablation}%
  \vspace{-5mm}
\end{table}%


\textbf{I. Random Masked Sentence Prediction Pre-training}~
To explain the observed improvements, our first hypothesis is: Models harvest \textit{extra linguistic ability} from masked \textit{statement} prediction compared with masked \textit{token (or span)} prediction.
Quite intuitively, filling entire sentences with complete subject-predicate structures might put additional demands on models to capture more abundant syntactic information beyond the coverage of masked token (or span) prediction.
Since LogiGAN involves recovering masked \textbf{\textit{sentences}}, it is then necessary to determine to what degree, if any, that the observed performance gain is attributable to models' plausible linguistic ability improvement. 
We therefore carry out a variant pre-training where the prediction objects are \textit{randomly masked sentence}.


% Since logic reasoning are primarily dependent on linguistic abilities -- language as lower infrastructures, and logic reasoning as upper establishments -- our important first step will be to disentangle linguistic ability from logic ability.
 
Results (shown in Table \ref{tab:ablation}) displays that masked sentence prediction training barely brings improvement against the vanilla baseline.
This suggests it is unlikely that masked sentence prediction empowers PLM trained from masked token prediction significantly better linguistic ability, nor likely that the extra pre-training corpus per se significantly raises the performance.
Therefore, we reject the first hypothesis and conclude that observed improvements should derive from somewhere else.
% Accounting overlaps between BookCorpus and T5'native $750GB$ C4 corpus, as well as the low marginal benefits of $2GB$ extra pre-training corpus per se --
% the improvement should therefore derive elsewhere.

\textbf{II. MLE-only Logic Pre-training}~
Our second hypothesis is that logic-guided masked statement prediction enhances models' intrinsic ability of logical reasoning, thereby lifting the downstream performance.
Having addressed the potential impact of learning randomized complete sentence generation, we next aim to check how learning logic-targeted statement generation affects models' behavior.
We ablate the entire adversarial training process, and train models to perform maximum likelihood estimation (MLE) with teacher-forcing loss only on masked-out logical statements.

% Since logic indicators provides reliable marks for such logic phenomena, we argue training models to predict the statements after logic indicators has dual function by its nature:
% (i) a pure linguistic aspect that is also captured by random masked sentence prediction;
% (ii) an advanced reasoning logic aspect that is deeply embedded in the semantics, instead of the superficial grammar or syntax of these statements.
% Going beyond \textit{I - Random Masked Sentence Prediction Pre-training} that is designed to explore impact of (i), we here investigate the impact of (ii) through carrying out pure generative logic pre-training.


Results \ref{tab:ablation} of MLE-only logic pre-training reveals quite a notable improvement across almost all datasets against both vanilla baseline and I., suggesting that learning to generate logical statements indeed injects extra abilities into the model.
Since results of I. eliminate the possibility that models harvest stronger linguistic abilities from complete sentence prediction, it is safe to partially ascribe the better downstream performance to models' enhanced ability in modeling logical reasoning. 
This reveals the relative orthogonality between logic ability and models' inherent linguistic ability, suggesting that logic ability could be enhanced through further logic-targeted pre-training.
 
\textbf{III. Iterative Multi-task Pre-training}~
Since II. only partially explains the observed improvements, here is our last hypothesis: the adversarial training procedure of LogiGAN explains the unexplained rest part beyond the coverage of II.  
% This hypothesis seems plausible because critical discrimination logical coherency between premises and conclusions and conditional conceiving of logical from scratch appears to be distinctive from each other.
Here a multi-task pre-training with both generation and verification tasks will be the most natural intermediate setting between the \textit{single-model generation-only setting} of II. and LogiGAN's \textit{dual-model adversarial setting}. 
However, since the verification task relies on Generator's self-sampled statements, we adopt an iterative self-critic pre-training manner following \cite{nijkamp-etal-2021-script}.
Unlike typical multi-tasking training that simultaneously carries different tasks and then sums the losses,
our generation and verification tasks happen alternately
\footnote{Verification is formulated as a generation task -- model outputs natural language token ``good'' and ``bad''.}.
% After the initial warm-up just as done in GAN, the Generator produces exactly ONE answer for each training example from Verifier training corpus.
% The rest of the training is similar to the training process of GAN described in \ref{gan-train}.

Surprisingly, the iterative multi-task pre-training barely brings any positive effects to models' downstream performance compared with II.
One possible explanation for this might be that
the drastically different mechanisms between the verification and generations task intervene with each other,
making the single-model \& multi-task setting non-beneficial. 
Now that we have confirmed that an extra verification task fails to explain the rest improvement,
we can accept our final hypothesis and conclude that it is indeed the adversarial mechanism between the Generator and Verifier that truly facilitate learning of logical reasoning, thereby further improving the downstream performance beyond II.




==> experiments_legacy.tex <==
\section{Experiments} \label{sec:experiments}

\subsection{Experiment Setup}
\subsubsection{Datasets}
To test the effectivenss of our pre-training approach,
we extensively experiment on $\mathbf{12}$ datasets. 
Two of our selected datasets focus specifically measuring models' logical reasoning ability: ReClor \citep{yu2020reclor}, LogiQA \citep{10.5555/3491440.3491941}. Apart from them, we also test with machine reading comprehension (MRC) datasets requiring deep understanding of natural language -- better logic ability could potentially assist this process, because deep understanding of passage usually necessitate reasoning and inference below the surface of words and sentences:
NarrativeQA \citep{narrativeqa},
QuoRef \citep{Dasigi2019QuorefAR},
RACE \citep{lai2017large},
DREAM \citep{sundream2018},
adversarial NLI - aNLI \citep{DBLP:journals/corr/abs-1910-14599}.


LogiGAN does not inject specialized knowledge such as mathematics or tabular understanding. Thus, we are not experimenting with reasoning requiring extra premises and limit our scope to tasks testing general reasoning abilities.

\subsubsection{Implementation Details}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/corpus-stat.pdf}
    \caption{Corpus statistics.}
    \label{fig:overview}
    % \vspace{-3mm}
\end{figure*}
\textbf{Pre-train Corpus Details}~~
We apply the corpus construction methodology (section \ref{sec:corpus}) on \textit{BookCorpus} \citep{soskkobayashi2018bookcorpus}, which consists of web-scrawled e-books and movies with topics from general domains.
Although some corpus featuring debates and arguments \citep{walker-etal-2012-corpus, Abbott2016InternetAC, swanson-etal-2015-argument} appears to be more suitable for our logic pre-training focus, we did not elect them due to their high domain specificity in fields such as politics, law, and economics.
After heuristic filtering (e.g., to discard overly short statements, ``since'' indicating time rather than premises,  ``so'' indicating degree rather than conclusions), we are able to obtain totally $7.31$ million ($1.14$ million from conclusion indicators, $1.17$ million from premise indicators, $4.99$ million from contrast indicators) training examples.

\textbf{LogiGAN Details}~~
We randomly sample 2 million and 0.5 million for source training examples of Generator and Verifier, respectively, without replacement (i.e., $M = 2$ million, $N = 0.5$ million in Algorithm \ref{alg:training}). 
We then partition the source Generator training corpus into to two $1$ million subsets for warmup and GAN training (i.e., $M_\alpha = M_\beta = $ $1$ million). 
In each iteration of GAN training, $10\%$ or $0.1$ million and $0.05$ million examples are sampled for Generator and Verifier training (i.e., $m$ = $0.1$ million, $n$ = $0.05$ million). 
The warmup epoch $E$ is set to $5$, whereas the max number of GAN iteration is set to $10$.
For our main experiments, we initialize the $Generator$ from pre-trained ``google/t5-v1\_1-base'' or ``google/t5-v1\_1-large'', and the $Verifier$ as ``albert-large-v2'' from HuggingFace \citep{wolf-etal-2020-transformers}.
By default, our a
 
 \textbf{Downstream Details} We report 
 
 
\subsubsection{Downstream Baselines}
Since our pursuit is not to advance state-of-the-art results on the leaderboard, nor to introduce even more inductive bias or extra complexity to achieve some non-generalizable performance improvement, we only include comparable results into the comparison for fairness consideration.
Specifically, we report the pristine performance of various pre-trained language models that takes simplest input formats while solving the tasks in a purely end-to-end manner.



% Table generated by Excel2LaTeX from sheet '主实验'
% \begin{table}[htbp]

%   \centering
%   \resizebox{1.0\textwidth}{!}{
%     \begin{tabular}{ccccccccccccc}
%     \toprule
%     \multicolumn{2}{c}{Models/Dataset } & ReClor & LogiQA & RACE  & DREAM & QuoRef & Narrative QA & anli  & samsum & MuTual & xsum  & \multicolumn{1}{c|}{hotpotqa} \\
%     \midrule
%     \multicolumn{2}{c}{Vanilla T5$_{~base}$} & 35.2  & 27.19 & 63.89 & 59.36 & 70.76/74.58 & 48.11 & 44.1  & ?     & 67.38 & ?     & ? \\
%     \multicolumn{2}{c}{LogiGAN-ss$_{~base}$} & 40.2  & 34.72 & 67.13 & 63.38 & 75.02/78.68 & 49.44 & 49.5  & ?     & 69.41 & ?     & ? \\
%     \multicolumn{2}{c}{LogiGAN-es$_{~base}$} & 40    & 37.02 & 67.27 & 63.73 & 74.57/78.28 & 49.46 & 49.7  & ?     & ?     & ?     & ? \\
%     \midrule
%     \multicolumn{2}{c}{Vanilla T5$_{~large}$} & 44.2  & 41.01 & 78.99 & 78.98 & 80.06/83.25 & 50.31 & 58    & 41.4     & ?     & ?     & ? \\
%     \multicolumn{2}{c}{LogiGAN$_{~large}$} & 54.2  & ?     & 80.64 & 81.42 & 81.92/85.25 & ?     & 63.5  & 42.76 & ?     & 33.34 & ? \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Main results}
%   \label{tab:addlabel}
% \end{table}%

\textbf{IV. Replacing Self-Sampling with Retrieved Existing Sentences}

As we stated earlier in the artist analogy in section \ref{sec:analogy}, the Generator is shown with several possible generation results under a given context.
The source of these demonstrated example is variable -- they could either be endogenously sampled via beam search from the Generator's self distribution, or could be exogenously acquired via some external resources.
To explore the endogenous-exogenous deal, we carry our a variant version of GAN whose generator is trained with sentences retrieved by Elastic Search \cite{Gormley2015ElasticsearchTD}, rather than self-sampled sentences generated with checkpoint from last iteration.
Practically, our database consists of 3.6 million sentences discovered by the corpus construction process, and we keep top five similar retrieved sentences as training examples.

\subsection{Experiment Results}
% Table generated by Excel2LaTeX from sheet '主实验'
\begin{table}[htbp]
  \centering
  \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{cccccccc}
    \toprule
    \multicolumn{8}{c}{Multiple Choice \& Classification Datasets} \\
    \midrule
    \multicolumn{2}{c} {Models\,/\,Dataset} & ReClor & LogiQA & RACE  & DREAM & aNLI  & MuTual \\
    \multicolumn{2}{c}{\small Metrics} & {\small {\small $Acc$}}   & {\small {\small $Acc$}}   & {\small {\small $Acc$}} & {\small {\small $Acc$}} & {\small {\small $Acc$}} & {\small {\small $Acc$}} &
    \midrule
    \multicolumn{2}{c}{Vanilla T$5_{~base}$} & $35.20$ & $27.19$ & $63.89$ & $59.36$ & $44.10$ & $67.38$ \\
    \multicolumn{2}{c}{LogiGAN-ss$_{~base}$} & $40.20$ & $34.72$ & $67.13$ & $63.38$ & $49.50$ & $69.41$ \\
    \multicolumn{2}{c}{LogiGAN-es$_{~base}$} & $40.00$ & $37.02$ & $67.27$ & $63.73$ & $49.70$ & $69.98$ \\
    \midrule
    \multicolumn{2}{c}{Vanilla T$5_{~large}$} & $50.40$ & $38.56$ & $78.99$ & $78.98$ & $58.00$ & $76.41$ \\
    \multicolumn{2}{c}{LogiGAN$_{~large}$} & $54.80$ & $40.55$ & $80.67$ & $81.42$ & $63.50$ & $77.88$ \\
    \midrule
    \multicolumn{8}{c}{Generation Datasets} \\
    \midrule
    \multicolumn{2}{c} {Models\,/\,Dataset} & QuoRef & HotpotQA & NarrativeQA & TellMeWhy & SamSum & xSum \\
    \multicolumn{2}{c}{\small Metrics} & {\small {\small EM\,/\,F$_1$}} & {\small {\small EM\,/\,F$_1$}}  & {\small Rouge$_L$} & \small Rouge$_L$ & {\small Rouge$_L$} & {\small Rouge$_L$} \\
    \midrule
    \multicolumn{2}{c}{Vanilla T$5_{~base}$}  & $70.76$\,/\,$74.58$ & $61.11$\,/\,$74.86$ & $48.11$ & $30.03$ & $39.32$ & $29.14$ \\
    \multicolumn{2}{c}{LogiGAN-ss$_{~base}$} & $75.02$\,/\,$78.68$ & $62.68$\,/\,$76.14$ & $49.44$ & $31.18$ & $39.92$ & $30.26$ \\
    \multicolumn{2}{c}{LogiGAN-es$_{~base}$} & $74.94$\,/\,$78.40$ & $62.80$\,/\,$76.18$ & $49.46$ & $31.15$ & $40.21$ & $30.27$ \\
    \midrule
    \multicolumn{2}{c}{Vanilla T$5_{~large}$} & $80.06$\,/\,$83.25$ & $66.11$\,/\,$79.80$ & $51.09$ & $31.42$ & $41.40$ & $31.58$ \\
    \multicolumn{2}{c}{LogiGAN$_{~large}$} & $81.92$\,/\,$85.25$ & $67.04$\,/\,$80.36$ & $51.79$ & $32.72$ & $43.13$ & $33.49$ \\
    \bottomrule
    \end{tabular}}
  \label{tab:main}%
  \caption{Main Results}
\end{table}%





\subsection{Ablation Study and Analysis}

% Table generated by Excel2LaTeX from sheet 'Ablation'
\begin{table}[htbp]
  \centering
  \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{ccccccccc}
    \toprule
    \multicolumn{2}{c}{Models\,/\,Dataset} & ReClor & LogiQA & RACE  & DREAM & aNLI & QuoRef & NarrativeQA \\
    \multicolumn{2}{c}{\small Metrics} & {\small $Acc$}   & {\small $Acc$}   & {\small $Acc$}   & {\small $Acc$} & {\small $Acc$} & {\small EM\,/\,F$_1$} & {\small Rouge$_L$} \\
    \midrule
    \multicolumn{2}{c}{Vanilla T5$_{~base}$} & $35.20$  & $27.19$ & $63.89$ & $59.36$ & $44.10$ & $70.76$\,/\,$74.58$ & $48.11$ \\
    \multicolumn{2}{c}{LogiGAN-es$_{~base}$} & $40.20$  & $34.72$ & $67.13$ & $63.38$ & $49.40$ & $75.02$\,/\,$78.68$ & $49.44$ \\
    \midrule
    \multicolumn{2}{c}{I. Random Sentence} & $36.00$ & $30.56$ & $61.26$ & $58.15$ &  $45.40$ & $70.96$\,/\,$74.50$ & $48.38$  \\
    \multicolumn{2}{c}{II. MLE-only } & $38.80$  & $35.02$ & $64.55$ & $61.71$ & $46.00$ & $73.61$\,/\,$76.96$ & $49.30$ \\
    \multicolumn{2}{c}{III. Iterative Multi-task} & $37.20$  & $34.25$ & $64.01$ & $62.06$ & $46.20$ & $71.67$\,/\,$75.14$ & $49.15$ \\
    \bottomrule
    \end{tabular}}
 \caption{Ablation Studies}
  \label{tab:addlabel}%
\end{table}%




Having observed the significant performance enhancement brought by our full adversarial logic pre-training, we now aim to pinpoint the truly functional components of the training process through ablation studies, thereby deriving the origins of observed improvements.

\textbf{I. Random Masked Sentence Prediction Pre-training}
The first hypothesis to explain the performance enhancement: Models harvest additional linguistic ability from masked statement prediction compared with masked token prediction. 
Since logic reasoning are primarily dependent on linguistic abilities -- language as lower infrastructures, and logic reasoning as upper establishments -- our important first step will be to disentangle linguistic ability from logic ability.
Quite intuitively, filling statements that are complete with subject-predicate structures puts additional demands on models to capture more abundant syntactic information beyond the converge of masked token prediction.
Therefore, it is necessary to determine to what degree such linguistic ability enhancement through learning to model complete sentence, if any, empowers models trained from masked token prediction.
Practically, we random sample sentences from BookCorpus and carryout a random masked sentence prediction pre-training \textcolor{red}{Details}. 

With all downstream training and evaluation process kept unchanged from our main experiment, masked sentence models hardly demonstrates any performance improvement against the vanilla baseline.
This result provides evidence to reject the first hypothesis: models' performance improvement are not derived from better linguistic ability.

\textbf{II. MLE-only Logic Pre-training}
The second hypothesis to explain observed improvements: learning to model logic phenomena itself lifts the performance.
Recall we refer to writers' conclusion-drawing, explanation-making, and contrasting behavior as ``logic phenomena''.
Following this definition, since logic indicators provides reliable marks for such logic phenomena, we argue training models to predict the statements after logic indicators \textcolor{red}{I might later put this exposition to section 2.} has dual function by its nature:
(i) a pure linguistic aspect that is also captured by random masked sentence prediction;
(ii) a advanced reasoning logic aspect that is deeply embedded in the semantics, instead of the superficial grammar or syntax of these statements.
Going beyond \textit{I - Random Masked Sentence Prediction Pre-training} that is designed to explore impact of (i), we here investigate the impact of (ii) through carrying out pure generative logic pre-training.
The implementation is trivial: we simply ablate the GAN-loss from our full adversarial training, retaining only the teacher forcing loss.
All other hyper-parameters and training setting are held unchanged.

Results of pure generative logic pre-training reveals quite notable improvement across almost all datasets against both vanilla baseline and \textit{I}, suggesting that learning to model logic phenomena indeed brings model certain extra power.
Since the results from \textit{I} eliminates the possibility of stronger linguistic abilities, it is now safe to conclude that logic reasoning ability truly exists and plays an important role in determining models' performance across broad scope downstream tasks. This result close the first theme of our storyline: the ability of logic is beyond linguistics per se, and can be injected into language models via modeling logic phenomena. 

\textbf{III. Iterative Pre-training with the Verification Task}
The third hypothesis to explain observed improvements: the introduction of the additional verification task has auxiliary function in enhancing models' logic  ability beyond the scope of II. 
This hypothesis seems plausible because critical discrimination logical coherency between premises and conclusions and conditional conceiving of logical from scratch appears to be distinctive from each other.
Compared to the single task pure generative pre-training, a multi-task learning setting will be the most natural next step.
However, the most recently updated generator produces conclusion to be filled in the masked statements via self-sampling, we adopt an iterative self-critic pre-training manner following \cite{nijkamp-etal-2021-script}, where the Generator and Verifier shares all parameters, rather than a typical multi-tasking training via summation of two loss function.
\footnote{We  formulate the verification as a generation task -- model outputs ``good'' and ``bad'' in natural language.}
After the initial warm-up just as done in GAN, the Generator produces exactly ONE answer for each training example from Verifier training corpus.
The rest of the training is similar to the training process of GAN described in \ref{gan-train}.

Surprisingly, this training setting barely brings positive effects and even slightly harms models' downstream performance.
To eliminate the possibility of improper setting of training hyper-parameters, such as generator-verifier ratio of steps and learning rates, we extensively grid-search most combinations of parameter, yet still fail to elevate the performance.
However, a conclusion that the verification task is not effective at all contradicts the significant performance improvement observed in full-setting GAN compared with pure generative logic pre-training.
Thus, an eclectic conclusion will be that the drastically different mechanism verification task and generation task might intervene each other, and sharing parameters between Generator and Verifier is likely to be a bad design choice.
 

\subsection{Few-shot Experiments}



% Table generated by Excel2LaTeX from sheet 'Few-shot'
\begin{table}[htbp]
  \centering
  \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{ccccccccccc}
    \toprule
    \multicolumn{2}{c}{Models/Datasets} & RACE  & DREAM & ReCLor & LogiQA & aNLI  & NarrativeQA & $\alpha$NLG  & xsum  & samsum \\
    \multicolumn{2}{c}{\small metrics} & {\small $Acc$}  & {\small $Acc$} & {\small $Acc$}  & {\small $Acc$} & {\small $Acc$} & {\small Rouge$_L$} & {\small Rouge$_L$} & {\small Rouge$_L$} & {\small Rouge$_L$} \\
    \midrule
    \multicolumn{2}{c}{Vanilla T$5_{~base}$} & $25.27$ & $34.09$ & $26.20$ & $23.34$ & $33.50$ & $5.86$ & $10.90$ & $13.67$ & $13.52$ \\
    \multicolumn{2}{c}{I. Random Sentence} & $25.26$ & $32.50$  & $26.80$ & $25.03$ & $33.70$ & $16.79$ & $18.28$ & $15.39$ & $26.52$ \\
    \multicolumn{2}{c}{LogiGAN-es$_{~base}$} & $26.28$ & $35.05$ & $28.40$  & $26.57$ & $35.60$ & $18.83$ & $20.80$  & $17.34$ & $27.93$ \\
    \bottomrule
    \end{tabular}}
    \caption{Few shot performance}
  \label{tab:addlabel}%
\end{table}%



To explore the impact of logic ability in resource-scare scenarios, we also carryout experiments few-shot setting.
For each dataset, we random select 32 samples and fine-tune until convergence.
Since in our masked statement pre-training, models learn to generate complete sentence, the output format therefore aligns more closely to to downstream generative tasks, which might play a decisive in a data-scare setting. 
Thus, to eliminate the potential performance improvement explained by such format alignment, we add the $I-Random Sentence$ pre-training into the comparison.
Results are shown in Table \ref{tab:few-shot}.

















% \begin{table}[htbp]
%   \centering
% \resizebox{0.8\textwidth}{!}{
%     \begin{tabular}{cccccccc}
%     \toprule
%     \multicolumn{2}{c} {Models\,/\,Dataset} & ReClor & LogiQA & RACE  & DREAM & aNLI  & MuTual \\
%     \multicolumn{2}{c}{\small Metrics} & {\small {\small $Acc$}}   & {\small {\small $Acc$}}   & {\small {\small $Acc$}} & {\small {\small $Acc$}} & {\small {\small $Acc$}} & {\small {\small $Acc$}} \\
%     \midrule
%     \multicolumn{2}{c}{Vanilla T$5_{~base}$} & $35.20$ & $27.19$ & $63.89$ & $59.36$ & $44.10$ & $67.38$ \\
%     \multicolumn{2}{c}{LogiGAN-ss$_{~base}$} & $40.20$ & $34.72$ & $67.13$ & $63.38$ & $49.50$ & $69.41$ \\
%     \multicolumn{2}{c}{LogiGAN-es$_{~base}$} & $40.00$ & $37.02$ & $67.27$ & $63.73$ & $49.70$ & $69.98$ \\
%     \midrule
%     \multicolumn{2}{c}{Vanilla T$5_{~large}$} & $44.20$ & $?$ & $78.99$ & $78.98$ & $58.00$ & $76.41$ \\
%     \multicolumn{2}{c}{LogiGAN$_{~large}$} & $54.80$ & $40.55$ & $80.67$ & $81.42$ & $63.50$ & $77.88$ \\
%     \bottomrule
%     \end{tabular}}
%   \label{tab:addlabel}
%     \caption{Main results on multiple choice datasets.}
% \end{table}%


% \begin{table}[htbp]
%   \centering
%     \resizebox{0.9\textwidth}{!}{
%     \begin{tabular}{cccccrcc}
%     \toprule
%     \multicolumn{2}{c} {Models\,/\,Dataset} & QuoRef & HotpotQA & NarrativeQA & \multicolumn{1}{c}{TellMeWhy} & SamSum & xSum \\
%     \multicolumn{2}{c}{\small Metrics} & {\small {\small EM\,/\,F$_1$}} & {\small {\small EM\,/\,F$_1$}}  & {\small Rouge$_L$} & \multicolumn{1}{c}{{\small Rouge$_L$}} & {\small Rouge$_L$} & {\small Rouge$_L$} \\
%     \midrule
%     \multicolumn{2}{c}{Vanilla T5$_{~base}$} & $70.76$\,/\,$74.58$ & $61.11$\,/\,$74.86$ & $48.11$ & \multicolumn{1}{c}{$30.03$} & $39.32$ & $29.14$ \\
%     \multicolumn{2}{c}{LogiGAN-ss$_{~base}$} & $75.02$\,/\,$78.68$ & $62.68$\,/\,$76.14$ & $49.44$ & \multicolumn{1}{c}{$31.18$} & $39.92$ & $30.26$ \\
%     \multicolumn{2}{c}{LogiGAN-es$_{~base}$} & $74.94$\,/\,$78.40$ & $62.80$\,/\,$76.18$ & $49.46$ & \multicolumn{1}{c}{$31.15$} & $40.21$ & $30.27$ \\
%     \midrule
%     \multicolumn{2}{c}{Vanilla T$5_{~large}$} & $80.06$\,/\,$83.25$ & $66.11$\,/\,$79.80$ & $51.09$ & \multicolumn{1}{c}{$31.42$} & $41.40$ & $31.58$ \\
%     \multicolumn{2}{c}{LogiGAN$_{~large}$} & $81.92$\,/\,$85.25$ & $67.04$\,/\,$80.36$ & $51.79$ &
%     \multicolumn{1}{c}{$32.72$} & $43.13$ & $33.34$ \\
%     \bottomrule
%     \end{tabular}}
%   \caption{Main results on generation datasets.}
%   \label{tab:addlabel}%
% \end{table}%



==> intro_legacy.tex <==
\section{Introduction} %%看不见我%%

Transformer architectures, powered by the attention mechanism \citep{NIPS2017_3f5ee243}, is springing up a new tide of artificial intelligence, bringing radical revolution to almost all sub-communities.
As a primary beneficiary, Pre-trained Language Models (PLMs) from the Natural Language Processing (NLP) community leverages the information expressiveness advantage of transformer architectures, becoming increasingly more competent at capturing diminutive contextualized linguistic variations.
A great line of pre-training research \citep{DBLP:journals/corr/abs-1810-04805, DBLP:journals/corr/abs-2005-14165, 2020t5},  is gradually conquers the complex nature of natural language, and PLMs are approaching human-level in diverse tasks and applications requiring sophisticated understanding of human language.

Despite the emerging fervor, researchers soon realize there is a bottleneck that is insurmountable via merely improving linguistic ability: models' incompetence in \textbf{reasoning}.
Following this, reasoning from  begins: Numerical reasoning \citep{Dua2019DROPAR}, commonsense reasoning \citep{sap-etal-2020-commonsense}, temporal Reasoning \citep{DBLP:journals/corr/abs-2010-12753}, multi-hop reasoning \citep{yang2018hotpotqa}, hybrid reasoning \citep{chen-etal-2020-hybridqa}, just to name a few.
This wide coverage of reasoning brings researchers both opportunities and challenges: While specialized research with high granularity and flexibility becomes possible, some nevertheless feel like touching a different part of an elephant, and it seems to be hard to connect the scattered dots into a insightful holistic picture.
\iffalse
% wanjun
{With endeavors to explore whether there exists  a fundamental ability that can potentially serve as the cornerstone and benefit these scattered reasoning tasks, we realize that \textbf{logical reasoning} may play this important role.}
\fi

%With endeavors to connect the dots, we realize that there is a specific type of reasoning that serves as the cornerstone for all reasoning, and remain invariant across most, if not all variations: logical reasoning.
While building a global connection is overly challenging, we do recognize 
With endeavors to connect the dots, we realize that \textbf{logical reasoning} serves as the cornerstone for all reasoning.
Reasoning is essentially an inferential process where an un-presented idea is drawn based on several presented ideas, and logic is the systemic set of rules for correctness guarantee of both the process per se and its product \citep{Hurley1982-HURACI}.
Regardless of the variability of concrete contents, logical reasoning has two essential invariant forms: draw conclusions based on some premises (aka. deduction \& induction, \cite{reichertz2013induction}), or hypothesize premises that explains some conclusions (aka. abduction \cite{sep-abduction}).
Setting aside the abductive reasoning task proposed by \cite{DBLP:journals/corr/abs-1908-05739}, existing variants of reasoning tasks in NLP can either be considered as 
(i) providing sufficient premises for drawing a conclusion but requiring specific way of premise extraction, such as multi-hop or hybrid reasoning;
or (ii) providing insufficient premises and requiring model to have external knowledge, such as commonsense or numerical reasoning.
\footnote{We expand our argument in depth in Appendix, and refer to intrigued readers there.}

However, discovering or invoking relevant premises is one thing, to produce proper conclusions based on such premises (i.e., reasoning logically) is another.
An abundance of neural-symbolic reasoning models, which first leverages PLMs to parse inputs into intermediate human-defined symbolic representations (i.e., generate premises), then outsources leftover reasoning steps to rule-based executors or specialized neural modules to assist production of final results.
This sheds light on PLMs' intrinsic lack of ability in logical reasoning. 







%%%%%%%%%%%%%%%%%%%%
 Learning should not be carried with a monolithic manner -- Critical thinking, or making reflective assessment and critique also plays a fundamental role.
 
 Our work makes both technical and intellectual contributions, not only to the computer science community -- the philosophical implications of our work could potentially bring insight to the field of cognitive modeling and educational psychology as well.
\begin{itemize}
    \item (Technical) We propose a novel GAN loss function design that is both differentiable and scalable to arbitrarily long output sequences.
    \item (Technical) We employ a self-supervised adversarial training manner to enhancement intrinsic logic reasoning ability of pre-trained language models.
    \item (Intellectual) We make the first formal attempt to disentangle logic ability from linguistic ability.
    \item (Intellectual) Our work provides evidence from a computational perspective for Confucius' renowned aphorism -- ``Learning without thought means labor lost; thought without learning is perilous", as well as the critical theory  \textcolor{red}{more details}.
\end{itemize}



==> intro_modified.tex <==
\section{Introduction} %%看不见我%%

Transformer architectures, powered by the attention mechanism \citep{NIPS2017_3f5ee243}, is springing up a new tide of artificial intelligence, bringing radical revolution to almost all sub-communities.
As a primary beneficiary, Pre-trained Language Models (PLMs) from the Natural Language Processing (NLP) community leverages the information expressiveness advantage of transformer architectures, becoming increasingly more competent at capturing diminutive contextualized linguistic variations.
A great line of pre-training research \citep{DBLP:journals/corr/abs-1810-04805, DBLP:journals/corr/abs-2005-14165, 2020t5},  is gradually conquers the complex nature of natural language, and PLMs are approaching human-level in diverse tasks and applications requiring sophisticated understanding of human language.

Despite the emerging fervor, researchers soon realize there is a bottleneck that is insurmountable via merely improving linguistic ability: models' incompetence in \textbf{reasoning}.
Following this, reasoning from  begins: Numerical reasoning \citep{Dua2019DROPAR}, commonsense reasoning \citep{sap-etal-2020-commonsense}, temporal Reasoning \citep{DBLP:journals/corr/abs-2010-12753}, multi-hop reasoning \citep{yang2018hotpotqa}, hybrid reasoning \citep{chen-etal-2020-hybridqa}, just to name a few.
This wide coverage of reasoning brings researchers both opportunities and challenges: While specialized research with high granularity and flexibility becomes possible, some nevertheless feel like touching a different part of an elephant, and it seems to be hard to connect the scattered dots into a insightful holistic picture.

{With endeavors to explore whether there exists  a fundamental ability that can potentially serve as the cornerstone and benefit these scattered reasoning tasks, we realize that \textbf{logical reasoning} may play this important role.}

Reasoning is essentially an inferential process where an un-presented idea is drawn based on several presented ideas, and logic is the systemic set of rules for correctness guarantee of both the process per se and its product \citep{Hurley1982-HURACI}.
Regardless of the variability of concrete contents, logical reasoning has two essential invariant forms: draw conclusions based on some premises (aka. deduction \& induction, \cite{reichertz2013induction}), or hypothesize premises that explains some conclusions (aka. abduction \cite{sep-abduction}).
Setting aside the abductive reasoning task proposed by \cite{DBLP:journals/corr/abs-1908-05739}, existing variants of reasoning tasks in NLP can either be considered as 
(i) providing sufficient premises for drawing a conclusion but requiring specific way of premise extraction, such as multi-hop or hybrid reasoning;
or (ii) providing insufficient premises and requiring model to have external knowledge, such as commonsense or numerical reasoning.
\footnote{We expand our argument in depth in Appendix, and refer to intrigued readers there.}

However, discovering or invoking relevant premises is one thing, to produce proper conclusions based on such premises (i.e., reasoning logically) is another.
An abundance of neural-symbolic reasoning models, which first leverages PLMs to parse inputs into intermediate human-defined symbolic representations (i.e., generate premises), then outsources leftover reasoning steps to rule-based executors or specialized neural modules to assist production of final results.
This sheds light on PLMs' intrinsic lack of ability in logical reasoning. 



%%%%%%%%%%%%%%%%%%%%
 Learning should not be carried with a monolithic manner -- Critical thinking, or making reflective assessment and critique also plays a fundamental role.
 
 Our work makes both technical and intellectual contributions, not only to the computer science community -- the philosophical implications of our work could potentially bring insight to the field of cognitive modeling and educational psychology as well.
\begin{itemize}
    \item (Technical) We propose a novel GAN loss function design that is both differentiable and scalable to arbitrarily long output sequences.
    \item (Technical) We employ a self-supervised adversarial training manner to enhancement intrinsic logic reasoning ability of pre-trained language models.
    \item (Intellectual) We make the first formal attempt to disentangle logic ability from linguistic ability.
    \item (Intellectual) Our work provides evidence from a computational perspective for Confucius' renowned aphorism -- ``Learning without thought means labor lost; thought without learning is perilous", as well as the critical theory  \textcolor{red}{more details}.
\end{itemize}



==> methodology.tex <==
\section{LogiGAN} %%看不见我%%

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/logiGAN.pdf}
    \caption{LogiGAN Overview.}
    \label{fig:overview}
    % \vspace{-3mm}
\end{figure*}

\subsection{Overview}
Similar to a typical conditional-GAN architecture, our adversarial training framework has two major components:
(i) a \textit{Generator} $\mathcal{G}$ that conditionally generate verisimilar examples to fool
(ii) the \textit{Verifier} $\mathcal{V}$ that learns to discriminate fake from real. 
Ideally, the more logically consistent a generated statement fit into the input context, the higher \textit{Verifier} truthfulness score it should receive. 
The  highest level optimization objective of LogiGAN can be expressed as \footnote{ We acknowledge that there is a gap between fake generated example and logically inconsistent examples, and explain further in details}:
\begin{equation}
\small
J^{\mathcal{G}^*.\mathcal{V}^*} = \min_{\mathcal{\theta}}\max_{\mathcal{\phi}} ~\mathbb{E}_{\bm{s}^+ \sim p_{\text{true}}(.|c)} [\log \mathcal{V}_{\phi}(c, \bm{s}^+)] + \mathbb{E}_{\bm{s^ -} \sim  p_{\text{neg}}(. | \mathcal{G}_\theta, c, s^+)} [\log (1 - \mathcal{V}_{\phi}(c, s^{-}))].
\end{equation}


\begin{algorithm}[t]
\caption{Adversarial Training Process} 
\label{alg:training}
% \small
\SetKwInOut{Input}{Dependencies}
\SetKwInOut{Output}{Output}
\Input{(1) A Pre-trained Generative Language Model as Generator $\mathcal{G}_0$\\
(2) A Pre-trained Discriminative Language Model as Verifier $\mathcal{V}_0$\\ 
(3) Generator Source Training Coprus $C_\mathcal{G}$ with size $M$\\
(4) Verifier Source Training Corpus $C_\mathcal{V}$ with size $N$\\
(5) Pre-defined Warmup epochs $E$, max iterations of GAN training $Q$\\
(6) Pre-defined training sample size $m$, $n$ for $\mathcal{G}$, $\mathcal{V}$ per iteration\\}

Random partition $C_\mathcal{G}$ into $C_{\mathcal{G}_\alpha}$, $C_{\mathcal{G}_\beta}$ with size $M_\alpha$, $M_\beta$;\\
$\mathcal{G}_0$ $\leftarrow$ Warmup $\mathcal{G}_\alpha$ on $C_{\mathcal{G}0}$ for $E$ epochs with $\mathcal{L}_{tf}$;\\
\For{i in  1:Q}{
    ${C_\mathcal{G}}_i \leftarrow$ Sample $m$ examples from $C_\mathcal{G_\beta}$ w/o replacement; \\
    ${C_\mathcal{V}}_i \leftarrow$ Sample $n$ examples from $C_\mathcal{V}$ w/o replacement;  \\
    $\widehat{{C_\mathcal{V}}_i} \leftarrow$  $\mathcal{G}_{i-1}$ do inference on ${C_\mathcal{V}}_i$;  \\
    $\widetilde{{C_\mathcal{G}}_i} \leftarrow$  $\mathcal{G}_{i-1}$ do inference on ${C_\mathcal{G}}_i$;  \\
    $\mathcal{V}_i \leftarrow$ Train  $\mathcal{V}_{i-1}$ on $\widehat{{C_\mathcal{V}}_i}$ for 1 epoch with $\mathcal{L}_{ver}$;\\
    $\widehat{{C_\mathcal{G}}_i} \leftarrow$  $\mathcal{V}_{i}$ do inference on $\widetilde{C_{\mathcal{G}}}_i$;  \\
    $\mathcal{G}_i \leftarrow$ Train  $\mathcal{G}_{i-1}$ on $\widehat{{C_\mathcal{G}}_i}$ for 1 epoch with $\mathcal{L}_{gen}$;\\
}
\end{algorithm}



\subsection{GAN-loss}   \label{sec:analogy}
Here we convey the fundamental intuition of our design of GAN-loss by drawing an analogy: Suppose there is an $100\%$ honest poet (i.e., a generative model) called G, who is well-trained for composing but not criticizing poems, and we wish to measure G's skills of poetry (i.e., ability of generating desirable content).
To serve this purpose, we sample various pre-defined themes or subject-matters (i.e., various textual context in corpus) and hope to see G's behavior under these themes.
Instead of requiring G to actually write a large batch of works from scratch and evaluate them one-by-one, we could instead show G some of existing works that is likely to fit into the given theme, either composed by G or by others poet, and demands G to \textbf{rank} the displayed works based on the his/her likelihood of producing something qualitatively and stylishly similar (i.e., compute likelihood).
The ranking provided by G is then checked against the ranking from the other authoritative art critic (i.e., Verifier score), the agreeableness of which will then serve an objective evaluation of G's poetry skills could be formed -- If G is good at poetry, then G should also be able to properly appreciate existing works.


Any pre-trained language models that can perform classification task as BERT \citep{DBLP:journals/corr/abs-1810-04805}, ALBERT \citep{DBLP:journals/corr/abs-1909-11942}, RoBERTa \citep{DBLP:journals/corr/abs-1907-11692} and BART \citep{DBLP:journals/corr/abs-1910-13461},  will be suitable for the role of Verifier. The binary classification loss for a single pair of input/statement/label $(x, s, y)$ of Verifier can be mathematically expressed as (omitting average):
\begin{equation}
    \small 
    \mathcal{L}_{ver}(x, s, y) = -y \log \mathcal{V}_\phi(y ~|~ [x; s]) - (1 - y) \log (1 - \mathcal{V}_\phi(y ~|~ [x; s]))
\end{equation}

where generated statements $s$ is either the top-k inference self-sampled from Generator given encoder input $x$ with $y = 0$, or the gold statement from original corpus with $y = 1$. 

For the purpose of smoothing gradient of GAN training process, it is usually a wise practice to gather both the positive and negative examples regarding a single input context $X$ inside the same batch. \textcolor{red}{reference}.
In our case, there is exactly one positive example and $n$ (we set $n = 5$) negative examples for each input context $x$.
For a batch of input/prediction pair $(x; s^+, s^{-}_1, ..., s^{-}_{n})$, our GAN-loss of Generator is designed for each batch of examples as: 
$$
\mathcal{L}_{gen} (x; s^+, s^{-}_1, ..., s^{-}_{n}) = \lambda_1 ~ \mathcal{L}_{tf}(x, s^+) + \lambda_2 ~ D_{KL} (\mathcal{G}_{\text{score}}(s^{-}_1, ..., s^{-}_{n}) ~||~ \mathcal{V}_{\text{score}}(s^{-}_1, ..., s^{-}_{n})),
$$
$$
\mathcal{G}_{\text{score}}(s^{-}_1, ..., s^{-}_{n}) = [ \ell_{\theta} (s^{-}_1 ~|~ c);~ \ell_{\theta} (s^{-}_2 ~|~ c);~ ...;~ \ell_{\theta} (s^{-}_n ~|~ c)],
$$
$$
\mathcal{V}_{\text{score}}(s^{-}_1, ..., s^{-}_{n}) = [ \mathcal{V}_{\phi} (s^{-}_1, c);~ \mathcal{V}_{\phi} (s^{-}_2, c);~ ...;~ \mathcal{V}_{\phi} (s^{-}_n, c)].  
$$


Our special design of GAN-loss circumvents the two most prickly issues in applying GAN-alike training on language models:
(i) the feedback from Verifier is not back-propagatable to Generator because of the intermediate non-differentiable beam-search mechanism for sentence generation; and
(ii) the intractable computational cost of Monte Carlo sampling for token-wise policy gradient estimation that grows exponentially with the length of output sequence.
Due to the computational infeasibility, the maximum output length of SeqGAN is capped at 5, whereas GAN-loss of our design could scale to arbitrarily long output sequences.
Wrapping things up, the overall iterative training process is described in Algorithm \ref{alg:training}. 
 \begin{equation}
p_{\text{neg}}(. ~|~ \mathcal{G}_\theta, c, s^+) = \{s_\alpha \sim G_\theta{(. ~|~ c)} ~~\cup~~ s_{{\small \beta}} \sim R(s^+)\} 
\end{equation}
where R is some retriever to obtain textually statements similar to $s^+$ but not necessarily to be logically consistent from external resources.



% Our special design of GAN-loss circumvents the two most prickly issues in applying GAN-alike training on language models:
% (i) the feedback from Verifier is not back-propagatable to Generator because of the intermediate non-differentiable beam-search mechanism for sentence generation; and
% (ii) the intractable computational cost of Monte Carlo sampling for token-wise policy gradient estimation that grows exponentially with the length of output sequence, as originally proposed in SeqGAN \cite{10.5555/3298483.3298649}.
% Due to the computational infeasibility, the maximum output length of SeqGAN is capped at 5, whereas GAN-loss of our design could scale to arbitrarily long output sequences.
% Wrapping things up, the overall iterative training process is described in Algorithm \ref{alg:training}. 
%  \begin{equation}
% p_{\text{neg}}(. ~|~ \mathcal{G}_\theta, c, s^+) = \{s_\alpha \sim G_\theta{(. ~|~ c)} ~~\cup~~ s_{{\small \beta}} \sim R(s^+)\} 
% \end{equation}
% where R is some retriever to obtain textually statements similar to $s^+$ but not necessarily to be logically consistent from external resources.


% \begin{equation}
% \small
% J^{\mathcal{G}^*.\mathcal{V}^*} = \min_{\mathcal{\theta}}\max_{\mathcal{\phi}} ~\mathbb{E}_{\bm{s}^+ \sim p_{\text{true}}(.|c)}[\log \mathcal{V}_{\phi}(c, \bm{s}^+)] + \mathbb{E}_{\bm{s^ -} \in {\{s_\alpha \sim \mathcal{G}_\theta(. | c) ~\cup~  ES(s^+) \}}}  [\log (1 - \mathcal{V}_{\phi}(c, s^{-}))].
% \end{equation}


